Observations of a radio-bright, X-ray obscured GRS 1915+105

The Galactic black hole transient GRS1915+105 is famous for its markedly variable X-ray and radio behaviour, and for being the archetypal galactic source of relativistic jets. It entered an X-ray outburst in 1992 and has been active ever since. Since 2018 GRS1915+105 has declined into an extended low-flux X-ray plateau, occasionally interrupted by multi-wavelength flares. Here we report the radio and X-ray properties of GRS1915+105 collected in this new phase, and compare the recent data to historic observations. We find that while the X-ray emission remained unprecedentedly low for most of the time following the decline in 2018, the radio emission shows a clear mode change half way through the extended X-ray plateau in 2019 June: from low flux (~3mJy) and limited variability, to marked flaring with fluxes two orders of magnitude larger. GRS1915+105 appears to have entered a low-luminosity canonical hard state, and then transitioned to an unusual accretion phase, characterised by heavy X-ray absorption/obscuration. Hence, we argue that a local absorber hides from the observer the accretion processes feeding the variable jet responsible for the radio flaring. The radio-X-ray correlation suggests that the current low X-ray flux state may be a signature of a super-Eddington state akin to the X-ray binaries SS433 or V404 Cyg.

==> A radio-active, X-ray obscured GRS 1915+105/def_bibtex.tex <==
\def\apj{ApJ}
\def\apjs{ApJ}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\apjl{ApJ}
\def\pasj{PASJ}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\skytel{S\&T}
\def\aaps{A\&A S.S.}
\def\araa{Annual Reviews}
\def\apss{Ap\&SS}
\def\atel{The Astronomer's Telegram}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\ssr{Space Science Reviews}
\def\prd{Physical Review D}
\def\pasp{Publications of the Astronomical Society of the Pacific}
\def\na{New Astronomy}

==> def_bibtex.tex <==
\def\apj{ApJ}
\def\apjs{ApJ}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\apjl{ApJ}
\def\pasj{PASJ}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\skytel{S\&T}
\def\aaps{A\&A S.S.}
\def\araa{Annual Reviews}
\def\apss{Ap\&SS}
\def\atel{The Astronomer's Telegram}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\ssr{Space Science Reviews}
\def\prd{Physical Review D}
\def\pasp{Publications of the Astronomical Society of the Pacific}
\def\na{New Astronomy}
